Is First Person Vision Challenging for Object Tracking?

Understanding human-object interactions is fundamental in First Person Vision (FPV). Tracking algorithms which follow the objects manipulated by the camera wearer can provide useful cues to effectively model such interactions. Despite a few previous attempts to exploit trackers in FPV applications, a methodical analysis of the performance of state-of-the-art visual trackers in this domain is still missing. In this short paper, we provide a recap of the first systematic study of object tracking in FPV. Our work extensively analyses the performance of recent and baseline FPV trackers with respect to different aspects. This is achieved through TREK-150, a novel benchmark dataset composed of 150 densely annotated video sequences. The results suggest that more research efforts should be devoted to this problem so that tracking could benefit FPV tasks. The full version of this paper is available at arXiv:2108.13665.

==> conclusions.tex <==
\section{Conclusions}
In this paper, we \AF{proposed} the first systematic evaluation of visual object tracking in FPV. The analysis \AF{has been} conducted with standard and novel measures on the newly introduced \datasetname\ benchmark, \AF{which} contains 150 video sequences extracted from the EK-55 \cite{EK55} FPV dataset. \datasetname\ has been densely annotated with 97K bounding-boxes, 17 sequence attributes, 
\AF{20 action verb attributes and 34 target object attributes.}
The performance of 31 state-of-the-art visual trackers and two baseline FPV trackers was analysed extensively on the proposed dataset. The results show a generalized drop in accuracy with respect to the \AF{performance} achieved on existing tracking benchmarks. \AF{Furthermore, our analysis provided} insights about which scenarios and actions cause the performance to change. Finally, we \AF{have shown} that object tracking gives an advantage in terms of \AF{object localization} accuracy and efficiency \AF{over} object detection.
\AF{These results suggest that FPV is a challenging scenario for current trackers and that tracking will likely get more importance in this domain as new FPV-specific solutions will be investigated.}
Annotations, results, and code, are available at \datasetlink.

==> relatedwork.tex <==
\input{tables/datasets.tex}

\section{Related Work}

\pgraph{Visual Tracking in FPV.}
\label{sec:fpvtrackers}
There have been some attempts to tackle visual tracking in FPV.
Alletto et al.~\cite{Alletto2015} improved the TLD tracker~\cite{TLD} with a 3D odometry based module to track people.
For a similar task, Nigam et al.~\cite{Nigam2017} proposed a combination of the Struck~\cite{Struck} and MEEM~\cite{MEEM} trackers with a person re-identification module.
Face tracking was tackled by Aghaei et al. \cite{Aghaei2016} through %
\AF{a}
multi-object tracking approach 
\AF{termed}
extended-bag-of-tracklets.
Hand tracking was studied in 
\AF{several}
works\AF{~\cite{kapidis2019egocentric,Visee2020,Mueller2017,Han2020,Sun2010}}. Sun et al. \cite{Sun2010} developed a particle filter framework for hand pose tracking. M{\"u}ller et al. \cite{Mueller2017} proposed a solution based on an RGB camera and a depth sensor. Kapidis et al. \cite{kapidis2019egocentric} and Vis\'ee et al. \cite{Visee2020} proposed to combine the YOLO \cite{YOLO} detector trained for hand detection with trackers. The
\AF{former}
used the multi-object tracker DeepSORT~\cite{DeepSORT}, whereas the 
\AF{latter}
employed the KCF \cite{KCF} single object tracker. Han et al. \cite{Han2020} exploited a detection-by-tracking approach on video frames acquired with 4 fisheye cameras.
All the presented solutions focused on tracking specific targets (i.e., people, faces, or hands), and thus they \AF{are likely to} fail in generalizing to arbitrary target objects. 
Moreover, they have been validated on custom designed datasets, \AF{which limits their reproducibility and the ability to compare them to other works}. 
\AF{In contrast,} we focus on the evaluation of algorithms \AF{for the generic object tracking task}.
\AF{We design our evaluation to be reproducible and extendable by releasing \datasetname, a dataset of 150 videos of different objects manipulated by the camera wearer, which we believe will be useful to study object tracking in FPV.}
To the best of our knowledge, 
\AF{ours is the first attempt}
to evaluate systematically generic object tracking in \AF{the FPV context}.







\pgraph{Visual Tracking for Generic Settings.}
In recent years, there has been an increased interest in developing accurate and robust single object tracking (SOT) algorithms for generic targets and domains.
Preliminary trackers were based on mean shift algorithms~\cite{Comanciu2000}, key-point~\cite{Matrioska}, part-based methods \cite{LGT,OGT}, or SVM learning~\cite{Struck}. Later, \AF{solutions based on} correlation filters gained popularity thanks to their processing speed~\cite{MOSSE,KCF,DSST,Staple,BACF}. More recently, \AF{algorithms based on} deep learning have been \AF{proposed} to extract efficient image and object features. This kind of representation has been used in deep regression networks~\cite{GOTURN,Dunnhofer2021ral}, online tracking-by-detection methods~\cite{MDNet,VITAL}, \AF{approaches} based on reinforcement learning~\cite{Yun2017,Chen2018,Dunnhofer2019,Guo2020tip}, deep discriminative correlation filters~\cite{ECO,ATOM,DiMP,PrDiMP,D3S,KYS}, and \AF{trackers based on} siamese networks~\cite{SiamFC,SiamRPNpp,SiamMask,SiamBAN,Ocean}. 
All these methods have been designed for tracking arbitrary target objects in unconstrained domains. However, no solution has been studied and validated on a number of diverse FPV sequences \AF{as} we propose in this paper.

\begin{figure*}[t]%
\centering
\includegraphics[width=\linewidth]{images/distributions.pdf}
\caption{(a) Distribution of the sequences within \datasetname\ with respect to the attributes. (b) Comparison of \AF{the} distributions \AF{of} common attributes \AF{in} different benchmarks. Distributions of (c) action verb labels, and (d) target object categories (nouns).}
\label{fig:distributions}
\vspace{-1.15em}
\end{figure*}

\pgraph{Visual Tracking Benchmarks.}
Disparate bounding box level benchmarks are available today to evaluate the performance of SOT algorithms. 
The Object Tracking Benchmarks (OTB) OTB-50 \cite{OTB2013} and OTB-100 \cite{OTB} are two of the most popular benchmarks in the visual tracking community. They provide 51 and 100 sequences respectively \AF{including} generic targets like vehicles, people, faces, toys, characters, etc.
The Temple-Color 128~(TC-128) dataset \cite{TC128} comprises 128 videos and was designed for the evaluation of color-enhanced trackers. 
The UAV123 dataset \cite{UAV123} was constructed to benchmark the tracking of 9 classes of target in 123 videos captured by unmanned aerial vehicle (UAV) cameras.
The NUS-PRO dataset~\cite{NUSPRO} contains 365 sequences and aims to benchmark human and rigid object tracking with targets belonging to one of 8 categories.
The Need for Speed (NfS) dataset~\cite{NfS} provides 100 sequences with a frame rate of 240 FPS. The aim of the authors was to benchmark the effects of frame rate variations on the tracking performance.
The VOT2019 benchmark~\cite{VOT2019} was the last iteration of the annual Visual Object Tracking challenge that required bounding-boxes as target object representation. This dataset contains 60 highly challenging videos, with generic target objects belonging to 30 different categories. 
The Color and Depth Tracking Benchmark (CDTB) dataset \cite{CDTB} offers 80 RGB sequences paired with a depth channel. This benchmark aims to explore the use of depth information to improve tracking performance. 
Following the increased development of deep learning based trackers, large-scale generic-domain SOT datasets have been recently released~\cite{TrackingNet,GOT10k,LaSOT}. These include more than \AF{a} thousand videos normally split into training and test subsets. The evaluation protocol \AF{associated with} these sets requires the evaluation of the trackers after \AF{they have been trained on}
the provided training set.
Despite the fact that all the presented benchmarks offer various tracking scenarios, 
\AF{limited work has focused on FPV, with some studies tackling the problem of tracking pedestrians or cars from a moving camera~\cite{sanchez2019predictor}.}
\AF{Some datasets of egocentric videos such as ADL~\cite{pirsiavash2012detecting} and EK-55~\cite{EK55} contain bounding-box object annotations. But due to the sparse nature of such annotations (typically 1/2 FPS), these datasets cannot be used for the accurate evaluation of trackers in FPV context.}
To the best of our knowledge, our proposed \datasetname\ dataset is the first benchmark for tracking objects \AF{which are relevant to (or manipulated by) a camera wearer} in egocentric videos. We believe that \datasetname\ is tantalizing for the tracking community because it offers complementary tracking situations (\AF{which we characterize}
with a total of $17$ attributes) and new target object categories (for a total of $34$) that are not present in other tracking benchmarks. 
Since in this paper we aim to benchmark generic approaches to visual tracking (that would not necessarily \AF{consider the} deep learning approach), we follow the practice of \AF{previous works} \cite{OTB,TC128,UAV123,NUSPRO,NfS,VOT2019,CDTB} and set up a well described dataset for evaluation of generic SOT algorithms. We believe that \datasetname\ can be a useful research tool for both the FPV and visual tracking research communities.


==> tables/datasets.tex <==
\begin{table*}[t]
\fontsize{8}{9}\selectfont
	\centering
	\caption{Statistics of the proposed \datasetname\ benchmark compared with other benchmarks designed for SOT evaluation.}
	\label{tab:datasets}
	\begin{tabular}{l | c  c  c  c  c  c  c  c | c }
		\toprule
		\multirow{2}{*}{Benchmark} & OTB-50 & OTB-100 & TC-128 & UAV123  & NUS-PRO & NfS  & VOT2019 & CDTB  & \multirow{2}{*}{\datasetname}\\
                    & \cite{OTB2013} & \cite{OTB} & \cite{TC128} & \cite{UAV123}  & \cite{NUSPRO} & \cite{NfS}  & \cite{VOT2019} & \cite{CDTB}  \\
		\midrule
		\# videos & 51 & 100 & 128 & 123 & 365 & 100 & 60 & 80 & 150 \\
		\# frames & 29K & 59K & 55K & 113K & 135K & 383K & 20K & 102K & 97K \\
		Min frames \AF{across videos} & 71 & 71 & 71 & 109 & 146 & 169 & 41 & 406 & 161  \\
		Mean frames \AF{across videos} & 578 & 590 & 429 & 915 & 371 & 3830 & 332 & 1274 & 649 \\
		Median frames \AF{across videos} & 392 & 393 & 365 & 882 & 300 & 2448 & 258 & 1179 & 484 \\
		Max frames \AF{across videos} & 3872 & 3872 & 3872 & 3085 & 5040 & 20665 & 1500 & 2501 & 4640 \\
		Frame rate & 30 FPS & 30 FPS & 30 FPS  & 30 FPS  & 30 FPS  & 240 FPS  & 30 FPS  & 30 FPS  & 60 FPS  \\
		\# target object classes & 10 & 16 & 27  & 9  & 8 & 17  & 30  & 23  & 34  \\
		\# sequence attributes & 11 & 11 & 11 & 12  & 12 & 9 & 6  & 13  & 17  \\
		FPV & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \xmark & \cmark \\
		\# action verbs & n/a & n/a & n/a & n/a & n/a & n/a & n/a & n/a & 20 \\
		\bottomrule		
\end{tabular}
\end{table*}
